Optimizing Tail Latency in Commodity Datacenters using Forward Error Correction

Long tail latency of short flows (or messages) greatly affects user-facing applications in datacenters. Prior solutions to the problem introduce significant implementation complexities, such as global state monitoring, complex network control, or non-trivial switch modifications. While promising superior performance, they are hard to implement in practice. This paper presents CloudBurst, a simple, effective yet readily deployable solution achieving similar or even better results without introducing the above complexities. At its core, CloudBurst explores forward error correction (FEC) over multipath - it proactively spreads FEC-coded packets generated from messages over multipath in parallel, and recovers them with the first few arriving ones. As a result, CloudBurst is able to obliviously exploit underutilized paths, thus achieving low tail latency. We have implemented CloudBurst as a user-space library, and deployed it on a testbed with commodity switches. Our testbed and simulation experiments show the superior performance of CloudBurst. For example, CloudBurst achieves 63.69% and 60.06% reduction in 99th percentile message/flow completion time (FCT) compared to DCTCP and PIAS, respectively.

==> sec/analysis.tex <==
\section{Analysis}\label{sec:math}
In this section we show that \sys is complementary to existing low latency proposals. Given any per-packet latency distribution, \sys always reduce the 99th percentile (tail) latency.


% \subsection{Low latency}
Consider the following scenario: an message of $k$ packets is to be delivered from a sender, $S$, to a receiver, $D$. Using FEC code of rate $s$, $(s>1)$, the $k$ packets generated $k\cdot s$ encoded symbols. For rateless codes, we define $s$ as the eventual coding rate, which is the number of packets received before full recovery over $k$.
% Suppose there are $n$ paths between $(S,D)$, and 
The cumulative density function (CDF) for the per-packet latency of the paths in DCN is $F_{P}(\cdot)$. 
The 99th percentile latency is denoted as $T_{99}$, where $F_P(T_{99}) = 0.99$.

% First we consider the message is delivered over multipath over ECMP. Denote the latency distribution of ECMP in this scenario as $F_{ECMP}(\cdot)$, and the 99th percentile latency as $T_{ECMP}$. Since ECMP picks a path for the message flow uniformly in random, $F_P(\cdot)$ and $F_{ECMP}(\cdot)$ are the same, thus $T_{ECMP} = T_{P}$.

% Then we consider \sys in the same scenario. The joint distribution of the order statistics of an absolutely continuous distribution
We compare the average per packet latency for \sys, and the 99th percentile tail packet latency for \sys.

Assume $F_X$ is absolutely continuous, it has a density such that $d F_X(x)=f_X(x) dx$, and we can use the substitutions
$u=F_X(x)$
and
$du=f_X(x)\,dx$
to derive the following probability density functions (pdfs) for the order statistics of a sample of size $k\cdot s$ drawn from the distribution of $X$:

\[f_{X_{(k)}}(x) =\frac{n!}{(k-1)!(n-k)!}F_X(x)^{k-1}[1-F_X(x)]^{n-k} f_X(x)\]
%\[
%\begin{aligned}
%	&f_{X_{(j)},X_{(k)}}(x,y)&=&\frac{n!}{(j-1)!(k-j-1)!(n-k)!}F_X(x)^{j-1}\cdot\\
%	& & &[F_X(y)-F_X(x)]^{k-1-j}[1-F_X(y)]^{n-k}\cdot\\
%	& & &f_X(x)f_X(y)
%\end{aligned}
%\]
%where $x\le y$
%
%\[f_{X_{(1)},\ldots,X_{(n)}}(x_1,\ldots,x_n)=n!f_X(x_1)\cdots f_X(x_n)\] 
%where $x_1\le x_2\le \dots \le x_n.$

